Robust Self-Supervised Extrinsic Self-Calibration

Autonomous vehicles and robots need to operate over a wide variety of scenarios in order to complete tasks efficiently and safely. Multi-camera self-supervised monocular depth estimation from videos is a promising way to reason about the environment, as it generates metrically scaled geometric predictions from visual data without requiring additional sensors. However, most works assume well-calibrated extrinsics to fully leverage this multi-camera setup, even though accurate and efficient calibration is still a challenging problem. In this work, we introduce a novel method for extrinsic calibration that builds upon the principles of self-supervised monocular depth and ego-motion learning. Our proposed curriculum learning strategy uses monocular depth and pose estimators with velocity supervision to estimate extrinsics, and then jointly learns extrinsic calibration along with depth and pose for a set of overlapping cameras rigidly attached to a moving vehicle. Experiments on a benchmark multi-camera dataset (DDAD) demonstrate that our method enables self-calibration in various scenes robustly and efficiently compared to a traditional vision-based pose estimation pipeline. Furthermore, we demonstrate the benefits of extrinsics self-calibration as a way to improve depth prediction via joint optimization.

==> figures/both_qualitative.tex <==


\begin{figure*}[t!]
\centering
\subfloat{
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_01-rgb_7_04131fb1.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_05-rgb_7_89a852c0.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_06-rgb_7_0935301b.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_07-rgb_7_851143ac.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_08-rgb_7_2fff9472.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_09-rgb_7_570fd51a.png}
}
\vspace{-4mm}
\\
\subfloat{
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_01-inv_depth_7_fda4f2df.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_05-inv_depth_7_2bca48a2.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_06-inv_depth_7_40721199.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_07-inv_depth_7_ee4b9656.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_08-inv_depth_7_262042e2.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_09-inv_depth_7_9a32b507.png}
}
\vspace{-4mm}
\\
\subfloat[\emph{DDAD}]{
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_01-calc_normals_7_c7875beb.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_05-calc_normals_7_11c2267c.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_06-calc_normals_7_4d9ba474.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_07-calc_normals_7_338b1655.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_08-calc_normals_7_2ff0a179.png}
\includegraphics[width=0.16\linewidth]{images/ddad_qualitative/ddad-val-lidar-camera_09-calc_normals_7_8df871f3.png}
}
//
\subfloat{
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front-1480-rgb_1_40020b22.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back-1480-rgb_1_58b133e3.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_left-1480-rgb_1_be6332ab.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_right-1480-rgb_1_b91f6249.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_left-1480-rgb_1_ee63df59.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_right-1480-rgb_1_404be6c3.png}
}
\vspace{-4mm}
\\
\subfloat{
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front-1480-inv_depth_1_fc5d9c74.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back-1480-inv_depth_1_e7a451aa.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_left-1480-inv_depth_1_14718541.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_right-1480-inv_depth_1_556ac75b.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_left-1480-inv_depth_1_36184bc7.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_right-1480-inv_depth_1_66474543.png}
}
\vspace{-4mm}
\\
\subfloat[\emph{nuScenes}]{
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front-1480-calc_normals_1_74bf4dcd.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back-1480-calc_normals_1_9194d541.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_left-1480-calc_normals_1_2e9b09c7.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_right-1480-calc_normals_1_7e5eaccc.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_left-1480-calc_normals_1_b3d8e70b.png}
\includegraphics[width=0.16\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_right-1480-calc_normals_1_a356d291.png}
}
\caption{\textbf{Self-Supervised depth estimation results} on the \emph{DDAD} and \emph{nuScenes} datasets using our proposed method, including surface normals calculated from the predicted depth maps.}
\label{fig:ddad_qualitative}
\end{figure*}


==> figures/camviz.tex <==


\begin{figure*}[t!]
    \vspace{-3mm}
    \centering
    \subfloat[DDAD]{
    \includegraphics[width=0.45\linewidth,height=3.6cm]{images/pred_pcl_ddad_small.jpg}
    }
    \subfloat[NuScenes]{
    \includegraphics[width=0.45\linewidth,height=3.6cm]{images/pred_pcl_nuscenes_small.jpg}
    }
    % \vspace{-2mm}
    \caption{\textbf{Predicted pointclouds using FSM on the \textit{DDAD} and \textit{nuScenes} datasets}. For each dataset, the same network is used in all six images, predicted depth maps are lifted to 3D using camera intrinsics and extrinsics, and then combined \emph{without any post-processing}. As a way to visualize camera overlapping, we also show projected LiDAR points from adjacent views overlaid on each RGB image (this information is not used at training or test time).}
    \label{fig:camviz}
    % \vspace{-5mm}
\end{figure*}


==> figures/ddad_non_overlapping.tex <==

\begin{figure}[t!]
\centering
\subfloat{
\includegraphics[width=0.30\linewidth]{images/ddad_warps/1/rgb.png}
\includegraphics[width=0.30\linewidth]{images/ddad_warps/0/rgb.png}
\includegraphics[width=0.30\linewidth]{images/ddad_warps/2/rgb.png}
}
\vspace{-4mm}
\\
\subfloat{
\includegraphics[width=0.30\linewidth]{images/ddad_warps/1/rgb_context_1.png}
\includegraphics[width=0.30\linewidth]{images/ddad_warps/0/rgb_context_1.png}
\includegraphics[width=0.30\linewidth]{images/ddad_warps/2/rgb_context_1.png}
}
\vspace{-4mm}
\\
\subfloat{
\includegraphics[width=0.30\linewidth]{images/ddad_warps/1/mask_1_0_0.png}
\includegraphics[width=0.30\linewidth]{images/ddad_warps/0/mask_1_0_0.png}
\includegraphics[width=0.30\linewidth]{images/ddad_warps/2/mask_1_0_0.png}
}
\vspace{-4mm}
\\
\subfloat{
\includegraphics[width=0.30\linewidth]{images/ddad_warps/ddad_mask1.png}
\includegraphics[width=0.30\linewidth]{images/ddad_warps/ddad_mask0.png}
\includegraphics[width=0.30\linewidth]{images/ddad_warps/ddad_mask2.png}
}
\caption{\textbf{Non-overlapping masks} calculated on the \textit{DDAD} dataset. \textbf{First and second rows:} Target and context frames. \textbf{Third row:} Temporal mask from context to target. \textbf{Fourth row:} Spatial mask from surrounding target images.}
\label{fig:non_overlapping_masks}
\end{figure}


==> figures/ddad_qualitative.tex <==


\begin{figure*}[t!]
% \vspace{-2mm}
\centering
\subfloat{
\includegraphics[width=0.14\linewidth,height=1.4cm]{images/ddad_qualitative/ddad-val-lidar-camera_01-rgb_7_04131fb1.jpg}
\includegraphics[width=0.14\linewidth,height=1.4cm]{images/ddad_qualitative/ddad-val-lidar-camera_05-rgb_7_89a852c0.jpg}
\includegraphics[width=0.14\linewidth,height=1.4cm]{images/ddad_qualitative/ddad-val-lidar-camera_06-rgb_7_0935301b.jpg}
\includegraphics[width=0.14\linewidth,height=1.4cm]{images/ddad_qualitative/ddad-val-lidar-camera_07-rgb_7_851143ac.jpg}
\includegraphics[width=0.14\linewidth,height=1.4cm]{images/ddad_qualitative/ddad-val-lidar-camera_08-rgb_7_2fff9472.jpg}
\includegraphics[width=0.14\linewidth,height=1.4cm]{images/ddad_qualitative/ddad-val-lidar-camera_09-rgb_7_570fd51a.jpg}
}
\vspace{-4mm}
\\
\subfloat{
\includegraphics[width=0.14\linewidth,height=1.4cm]{images/ddad_qualitative/ddad-val-lidar-camera_01-inv_depth_7_fda4f2df.jpg}
\includegraphics[width=0.14\linewidth,height=1.4cm]{images/ddad_qualitative/ddad-val-lidar-camera_05-inv_depth_7_2bca48a2.jpg}
\includegraphics[width=0.14\linewidth,height=1.4cm]{images/ddad_qualitative/ddad-val-lidar-camera_06-inv_depth_7_40721199.jpg}
\includegraphics[width=0.14\linewidth,height=1.4cm]{images/ddad_qualitative/ddad-val-lidar-camera_07-inv_depth_7_ee4b9656.jpg}
\includegraphics[width=0.14\linewidth,height=1.4cm]{images/ddad_qualitative/ddad-val-lidar-camera_08-inv_depth_7_262042e2.jpg}
\includegraphics[width=0.14\linewidth,height=1.4cm]{images/ddad_qualitative/ddad-val-lidar-camera_09-inv_depth_7_9a32b507.jpg}
}
\\
% \subfloat{
% \includegraphics[width=0.14\linewidth,height=1.4cm,height=1.4cm]{images/ddad_qualitative/ddad-val-lidar-camera_01-calc_normals_7_c7875beb.jpg}
% \includegraphics[width=0.14\linewidth,height=1.4cm,height=1.4cm]{images/ddad_qualitative/ddad-val-lidar-camera_05-calc_normals_7_11c2267c.jpg}
% \includegraphics[width=0.14\linewidth,height=1.4cm,height=1.4cm]{images/ddad_qualitative/ddad-val-lidar-camera_06-calc_normals_7_4d9ba474.jpg}
% \includegraphics[width=0.14\linewidth,height=1.4cm,height=1.4cm]{images/ddad_qualitative/ddad-val-lidar-camera_07-calc_normals_7_338b1655.jpg}
% \includegraphics[width=0.14\linewidth,height=1.4cm,height=1.4cm]{images/ddad_qualitative/ddad-val-lidar-camera_08-calc_normals_7_2ff0a179.jpg}
% \includegraphics[width=0.14\linewidth,height=1.4cm,height=1.4cm]{images/ddad_qualitative/ddad-val-lidar-camera_09-calc_normals_7_8df871f3.jpg}
% }
% \vspace{-2mm}
\caption{
\textbf{Self-Supervised depth estimation results} using FSM on the \textit{DDAD} dataset.
}
% \vspace{-2mm}
%, including surface normals calculated from the predicted depth maps.}
\label{fig:ddad_qualitative}
\end{figure*}


==> figures/ddad_spatio_temporal.tex <==

\begin{figure}[t!]
\centering
\subfloat{
% \includegraphics[width=0.32\linewidth]{images/pd_warps/rgb2b.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/rgb4b.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/rgb5b.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/rgb1.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/rgb0.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/rgb2.png}
}
\vspace{-3.5mm}
\\
\subfloat{
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_2.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_4.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_5.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_1.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_0.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_2.png}
}
\vspace{-3.5mm}
\\
\subfloat{
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_context_2.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_context_4.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_context_5.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_context_1.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_context_0.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_context_2.png}
}
\caption{
\textbf{Examples of spatio-temporal photometric losses} on the \textit{DDAD} dataset. \textbf{Top row:} input RGB images. \textbf{Middle row:} Photometric losses considering only spatial contexts (Equation~\ref{eq:warp_spatial}). \textbf{Bottom row:} Photometric losses considering our proposed spatio-temporal contexts (Equation~\ref{eq:warp_multi}) from adjacent frames (forward and backwards).
}
\label{fig:pd_multicam}
\end{figure}


==> figures/ddad_warps.tex <==

\begin{figure*}[t!]
\centering
% \vspace{-5mm}
\subfloat{
\textcolor{green}{\rule{2.62cm}{1.5mm}}
\textcolor{cyan}{\rule{2.62cm}{1.5mm}}
\textcolor{magenta}{\rule{2.62cm}{1.5mm}}
\textcolor{yellow}{\rule{2.62cm}{1.5mm}}
\textcolor{red}{\rule{2.62cm}{1.5mm}}
\textcolor{blue}{\rule{2.62cm}{1.5mm}}
}
\vspace{-4.0mm}
\\
\subfloat{
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_photo/rgb3.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_photo/rgb1.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_photo/rgb0.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_photo/rgb2.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_photo/rgb4.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_photo/rgb5.jpg}
}
\vspace{-4.5mm}
\\
\subfloat{
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_photo/warp_self_3.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_photo/warp_self_1.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_photo/warp_self_0.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_photo/warp_self_2.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_photo/warp_self_4.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_photo/warp_self_5.jpg}
}
\vspace{-4.5mm}
\\
\subfloat{
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_viridis/3_photo_self_0_bwd.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_viridis/1_photo_self_0_fwd.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_viridis/0_photo_self_0_fwd.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_viridis/2_photo_self_0_fwd.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_viridis/4_photo_self_0_bwd.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_viridis/5_photo_self_0_bwd.jpg}
}
\vspace{-4.5mm}
\\
\subfloat{
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_photo2/warp_cross_3.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_photo2/warp_cross_1.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_photo2/warp_cross_0.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_photo2/warp_cross_2.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_photo2/warp_cross_4.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_photo2/warp_cross_5.jpg}
}
\vspace{-4.5mm}
\\ 
% \setcounter{subfigure}{1}
\subfloat{
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_viridis/3_photo_spatial_bwd.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_viridis/1_photo_spatial_bwd.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_viridis/0_photo_spatial_bwd.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_viridis/2_photo_spatial_bwd.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_viridis/4_photo_spatial_bwd.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_viridis/5_photo_spatial_bwd.jpg}
}
\vspace{-4.5mm}
\\ 
% \setcounter{subfigure}{1}
\subfloat{
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_viridis/3_photo_fsm_fwd.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_viridis/1_photo_fsm_fwd.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_viridis/0_photo_fsm_fwd.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_viridis/2_photo_fsm_fwd.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_viridis/4_photo_fsm_fwd.jpg}
\includegraphics[width=0.15\linewidth,height=1.4cm]{images/ddad_viridis/5_photo_fsm_bwd.jpg}
}
\caption{\textbf{Examples of spatial and temporal image warping} on the \textit{DDAD} dataset (camera colors from Figure~\ref{fig:teaser}, clockwise). \textbf{First row:} Input RGB images. \textbf{Second and third rows:} Synthesized views from temporal contexts (Equation~\ref{eq:warp_mono}) and photometric losses. \textbf{Fourth and fifth rows:} Synthesized views from surrounding cameras (Equation~\ref{eq:warp_spatial}), and photometric losses using only spatial contexts. \textbf{Sixth row} Photometric losses using our proposed spatio-temporal contexts. By also leveraging temporal contexts during cross-camera photometric warping, we are able to generate larger overlapping areas between images, as well as a smaller residual photometric error (darker colors) for optimization.}
\label{fig:ddad_warps}
% \vspace{-5mm}
\end{figure*}


==> figures/masking.tex <==


\begin{figure}[t!]
\centering
\subfloat[Input RGB image.]{
\includegraphics[width=0.48\linewidth,height=1.8cm]{images/ddad_warps/self_occlusion_rgb.jpg}
\label{fig:mask_rgb}
}
\subfloat[Self-occlusion mask.]{
\includegraphics[width=0.48\linewidth,height=1.8cm]{images/ddad_warps/cam_mask.jpg}
\label{fig:mask_binary}
}
\vspace{-3mm}
\\
\subfloat[Without self-occlusion masking.]{
\includegraphics[width=0.48\linewidth,height=1.8cm]{images/ddad_warps/self_occlusion_pre.jpg}
\label{fig:mask_without}
}
\subfloat[With self-occlusion masking.]{
\includegraphics[width=0.48\linewidth,height=1.8cm]{images/ddad_warps/self_occlusion_mask.jpg}
\label{fig:mask_with}
}
\caption{\textbf{Impact of self-occlusion masks on depth estimation} on the \textit{DDAD} dataset. These masks remove self-occluded regions from the self-supervised photometric loss, enabling easier optimization (lower loss, cf. Figure~\ref{fig:ddad_warps}) and better generalization (e.g., on the ground plane).}
\label{fig:self_occ_masks}
% \vspace{-3mm}
\end{figure}


% \begin{figure}[t!]
% \centering
% \subfloat{
% \includegraphics[width=0.22\textwidth]{images/pre_mask.jpg}
% }
% \subfloat{
% \includegraphics[width=0.22\textwidth]{images/cam_mask.jpg}
% }
% \caption{Same model before and after masking (top, left and right). The binary mask for this camera (bottom).}
% \end{figure}



==> figures/multicam_diagram.tex <==

\begin{figure}[t!]
    \centering
    \subfloat{
    \includegraphics[width=0.8\linewidth, height=4.0cm, trim=0 10 0 0, clip]{images/multicam_diagram3.png}
    }
    \caption{\textbf{Multi-camera spatio-temporal transformation matrices}. Solid cameras are \textit{target} (current frames), and dotted cameras are \textit{context} (adjacent frames). Spatial transformations ($\mathbf{X}_{i \rightarrow 1}$) are obtained from known extrinsics, and temporal transformations ($\hat{\mathbf{X}}^{\mathit{t} \rightarrow \mathit{c}}_i$) from the pose network.}
    \label{fig:multicam_diagram}
% \vspace{-3mm}
\end{figure}


==> figures/nuscenes_qualitative.tex <==


\begin{figure*}[t!]
% \vspace{-2mm}
\centering
\subfloat{
\includegraphics[width=0.14\linewidth, height=1.2cm]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front-1480-rgb_1_40020b22.jpg}
\includegraphics[width=0.14\linewidth, height=1.2cm]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back-1480-rgb_1_58b133e3.jpg}
\includegraphics[width=0.14\linewidth, height=1.2cm]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_left-1480-rgb_1_be6332ab.jpg}
\includegraphics[width=0.14\linewidth, height=1.2cm]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_right-1480-rgb_1_b91f6249.jpg}
\includegraphics[width=0.14\linewidth, height=1.2cm]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_left-1480-rgb_1_ee63df59.jpg}
\includegraphics[width=0.14\linewidth, height=1.2cm]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_right-1480-rgb_1_404be6c3.jpg}
}
\vspace{-4mm}
\\
\subfloat{
\includegraphics[width=0.14\linewidth, height=1.2cm]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front-1480-inv_depth_1_fc5d9c74.jpg}
\includegraphics[width=0.14\linewidth, height=1.2cm]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back-1480-inv_depth_1_e7a451aa.jpg}
\includegraphics[width=0.14\linewidth, height=1.2cm]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_left-1480-inv_depth_1_14718541.jpg}
\includegraphics[width=0.14\linewidth, height=1.2cm]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_right-1480-inv_depth_1_556ac75b.jpg}
\includegraphics[width=0.14\linewidth, height=1.2cm]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_left-1480-inv_depth_1_36184bc7.jpg}
\includegraphics[width=0.14\linewidth, height=1.2cm]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_right-1480-inv_depth_1_66474543.jpg}
}
\\
% \subfloat{
% \includegraphics[width=0.14\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front-1480-calc_normals_1_74bf4dcd.jpg}
% \includegraphics[width=0.14\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back-1480-calc_normals_1_9194d541.jpg}
% \includegraphics[width=0.14\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_left-1480-calc_normals_1_2e9b09c7.jpg}
% \includegraphics[width=0.14\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_right-1480-calc_normals_1_7e5eaccc.jpg}
% \includegraphics[width=0.14\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_left-1480-calc_normals_1_b3d8e70b.jpg}
% \includegraphics[width=0.14\linewidth]{images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_right-1480-calc_normals_1_a356d291.jpg}
% }
% \vspace{-2mm}
\caption{
\textbf{Self-Supervised depth estimation results} using FSM on the \textit{nuScenes} dataset.
}
% \vspace{-2mm}
%, including surface normals calculated from the predicted depth maps.}
\label{fig:nuscenes_qualitative}
\end{figure*}


==> figures/pcl_align.tex <==


\begin{figure}[t!]
    % \vspace{-4mm}
    \centering
    \subfloat[Monocular photometric loss (Abs Rel 0.211/0.241)]{
    \includegraphics[width=0.9\linewidth,height=2.5cm, trim=0 50 0 50, clip]{images/pcl_align_mono.jpg}
    }
\\
    % \vspace{-3mm}
    \subfloat[Spatio-temporal photometric loss (Abs Rel 0.201/0.207)]{
    \includegraphics[width=0.9\linewidth,height=2.5cm, trim=0 50 0 50, clip]{images/pcl_align_fsm.jpg}
    }
    % \vspace{-1mm}
    \caption{\textbf{Multi-camera pointcloud alignment} on DDAD using (a) the standard monocular photometric loss, and (b) our proposed spatio-temporal photometric constraints. We also report per-frame and shared median-scaling Abs Rel results (average of all cameras, see Table~\ref{tab:both_scaling_small} for more details).}
    % \vspace{-2mm}
    \label{fig:pcl_align}
% \vspace{-3mm}
\end{figure}


==> figures/pd_spatio_temporal.tex <==

\begin{figure}[t!]
\centering
\subfloat{
% \includegraphics[width=0.32\linewidth]{images/pd_warps/rgb2b.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/rgb4b.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/rgb5b.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/rgb1.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/rgb0.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/rgb2.png}
}
\vspace{-3.5mm}
\\
\subfloat{
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_2.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_4.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_5.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_1.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_0.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_2.png}
}
\vspace{-3.5mm}
\\
\subfloat{
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_context_2.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_context_4.png}
% \includegraphics[width=0.32\linewidth]{images/pd_warps/photo_cross_context_5.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_context_1.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_context_0.png}
\includegraphics[width=0.32\linewidth]{images/ddad_photo/photo_cross_context_2.png}
}
\caption{
\textbf{Examples of spatio-temporal photometric losses} on the \textit{DDAD} dataset. \textbf{Top row:} input RGB images. \textbf{Middle row:} Photometric losses considering only spatial contexts (Equation~\ref{eq:warp_spatial}). \textbf{Bottom row:} Photometric losses considering our proposed spatio-temporal contexts (Equation~\ref{eq:warp_multi}) from adjacent frames (forward and backwards).
}
\label{fig:pd_multicam}
\end{figure}


==> figures/pd_warps.tex <==

\begin{figure*}[t!]
\vspace{-5mm}
\begin{tabular}{cc}
\centering
\multirow{6}{*}{
\hspace{-3mm}
\subfloat[Camera locations on the vehicle.]{
\raisebox{-51mm}{\includegraphics[width=0.28\linewidth,trim=0 350 0 0, clip]{images/pd_6cams.png}}}}
\hspace{-5mm}
& 
\\
& 
\hspace{0.2mm}
\subfloat{
\textcolor{cyan}{\rule{1.93cm}{1mm}}
\textcolor{magenta}{\rule{1.92cm}{1mm}}
\textcolor{yellow}{\rule{1.92cm}{1mm}}
\textcolor{green}{\rule{1.92cm}{1mm}}
\textcolor{blue}{\rule{1.92cm}{1mm}}
\textcolor{red}{\rule{1.92cm}{1mm}}
}
\vspace{-4.5mm}
\\
& 
\hspace{0.1mm}
\subfloat{
\includegraphics[width=0.11\linewidth,height=1.0cm]{images/ddad_photo/rgb0.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/rgb1.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/rgb2.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/rgb3.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/rgb4.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/rgb5.png}
}
\vspace{-4.5mm}
\\
& 
\hspace{0.1mm}
\subfloat{
\includegraphics[width=0.11\linewidth]{images/ddad_photo/warp_self_0.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/warp_self_1.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/warp_self_2.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/warp_self_3.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/warp_self_4.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/warp_self_5.png}
}
\vspace{-4.5mm}
\\
& 
\hspace{0.1mm}
\subfloat{
\includegraphics[width=0.11\linewidth]{images/ddad_photo/photo_self_0.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/photo_self_1.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/photo_self_2.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/photo_self_3.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/photo_self_4.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo/photo_self_5.png}
}
\vspace{-4.5mm}
\\
& 
\hspace{0.1mm}
\subfloat{
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/warp_cross_0.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/warp_cross_1.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/warp_cross_2.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/warp_cross_3.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/warp_cross_4.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/warp_cross_5.png}
}
\vspace{-4.5mm}
\\ 
&
\setcounter{subfigure}{1}
\subfloat[\textbf{First row:} Input RGB images. \textbf{Second and third rows:} Synthesized views from temporal contexts (Equation~\ref{eq:warp_mono}) and the corresponding photometric losses. \textbf{Third and fourth rows:} Synthesized views from surrounding cameras (Equation~\ref{eq:warp_spatial}) and the corresponding photometric losses (both overlaid).]{
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/photo_cross_0.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/photo_cross_1.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/photo_cross_2.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/photo_cross_3.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/photo_cross_4.png}
\includegraphics[width=0.11\linewidth]{images/ddad_photo2/photo_cross_5.png}
}
\end{tabular}
\caption{\textbf{Examples of spatial and temporal image warping} on the \textit{DDAD}  dataset. (a) shows the location of all six cameras, and (b) depicts the RGB images for each camera, alongside the synthesized images using information from other viewpoints and their corresponding photometric losses.}
\label{fig:pd_warps}
\vspace{-5mm}
\end{figure*}


==> figures/teaser.tex <==

\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{images/selffsm_teaser.png}
\caption{\textbf{Consistent scale-aware Full Surround Monodepth (FSM) pointcloud} from multiple cameras.}
%\caption{(This figure is a stand-in for the described figure). Consistent multi-camera depth estimation.  A single network is trained with our multi-camera constraints, yielding a consistent $360\degree$}
% \vspace{-5mm}
\label{fig:teaser}
% \vspace{-5mm}
\end{figure}


==> tables/both_scaling_small.tex <==

\begin{table}%
% \vspace{-1mm}
\centering
\small
\renewcommand{\arraystretch}{1.05}
\setlength{\tabcolsep}{0.3em}
\subfloat[DDAD]{
\begin{tabular}{l|c|cccccc}
    \toprule
    \multirow{2}{*}{} &
    \multirow{2}{*}{\rotatebox{90}{\textbf{Scaling}}} &
    \multicolumn{6}{c}{Abs.Rel.$\downarrow$} \\
    \cmidrule{3-8}
    & 
    & \textit{Front}
    & \textit{F.Left}
    & \textit{F.Right}
    & \textit{B.Left}
    & \textit{B.Right}
    & \textit{Back}
    \\
    \midrule
    Mono $-$ M
    & F
    & 0.184
    & 0.366
    & 0.448
    & 0.417
    & 0.426
    & 0.438
    \\
    Mono
    & F 
    & 0.139
    & 0.209
    & 0.236
    & 0.231
    & 0.247
    & 0.204
    \\
    \textbf{FSM}
    & F
    & \underline{0.131}
    & \underline{0.203}
    & \underline{0.226}
    & \textbf{0.223}
    & \textbf{0.240}
    & \underline{0.188}
    \\
    \midrule
    Mono
    & S
    & 0.143
    & 0.238
    & 0.265
    & 0.277
    & 0.276
    & 0.247
    \\
    \textbf{FSM}
    & S
    & 0.133
    & 0.212
    & 0.229
    & 0.231
    & \underline{0.246}
    & 0.194
    \\ 
    \midrule
    \textbf{FSM $-$ STC}
    & -
    & 0.133
    & 0.219
    & 0.246
    & 0.252
    & 0.259
    & 0.197
    \\
    \textbf{FSM $-$ PCC}
    & -
    & \underline{0.131}
    & 0.206
    & 0.228
    & 0.238 
    & 0.248
    & \underline{0.188}
    \\
    \textbf{FSM}
    & -
    & \textbf{0.130}
    & \textbf{0.201}
    & \textbf{0.224}
    & \underline{0.229}
    & \textbf{0.240}
    & \textbf{0.186}
    \\
    \bottomrule
\end{tabular}
}
\\
\vspace{-2mm}
\subfloat[nuScenes]{
\begin{tabular}{l|c|cccccc}
    \toprule
    \multirow{2}{*}{} &
    \multirow{2}{*}{\rotatebox{90}{\textbf{Scaling}}} &
    \multicolumn{6}{c}{Abs.Rel.$\downarrow$} \\
    \cmidrule{3-8}
    & 
    & \textit{Front}
    & \textit{F.Left}
    & \textit{F.Right}
    & \textit{B.Left}
    & \textit{B.Right}
    & \textit{Back}
    \\
    \midrule
    Mono
    & F 
    & 0.214
    & 0.304
    & 0.388
    & 0.314 
    & 0.438 
    & 0.304 
    \\
    \textbf{FSM}
    & F
    & 0.198
    & 0.297
    & \textbf{0.350}
    & \textbf{0.289} 
    & \textbf{0.392}
    & \underline{0.240}
    \\
    \midrule
    Mono
    & S
    & 0.251
    & 0.403 
    & 0.546
    & 0.429 
    & 0.616 
    & 0.321 
    \\
    \textbf{FSM}
    & S
    & 0.200 
    & 0.337 
    & 0.448
    & 0.354 
    & 0.521 
    & 0.267 
    \\ 
    \midrule
    \textbf{FSM $-$ STC}
    & -
    & 0.208
    & 0.382
    & 0.510
    & 0.393
    & 0.595
    & 0.258
    \\ 
    \textbf{FSM $-$ PCC}
    & -
    & \underline{0.187} 
    & \underline{0.291}
    & 0.392
    & 0.311
    & 0.448
    & 0.235
    \\ 
    \textbf{FSM}
    & -
    & \textbf{0.186}
    & \textbf{0.287}
    & \underline{0.375}
    & \underline{0.296}
    & \underline{0.418}
    & \textbf{0.221}
    \\
    \bottomrule
\end{tabular}
}
\vspace{-2mm}
\caption{\textbf{Depth estimation results on multi-camera datasets}, using \emph{FSM} relative to the single-camera photometric loss (\emph{Mono}). In the scaling column, \emph{F} denotes per-frame median-scaling, and \emph{S} our proposed shared median-scaling. \emph{M} denotes the removal of masking (Sec.~\ref{sec:mask}), \emph{STC} the removal of spatio-temporal contexts (Sec.~\ref{sec:stc}), and \emph{PCC} the removal of pose consistency constraints (Sec.~\ref{sec:pcc}).}
\label{tab:both_scaling_small}
\vspace{-3mm}
\end{table}

==> tables/both_scaling_small2.tex <==

\begin{table}%
% \vspace{-1mm}
\centering
\small
\renewcommand{\arraystretch}{1.00}
\setlength{\tabcolsep}{0.22em}
\subfloat[DDAD]{
\begin{tabular}{l|cccccc|c}
    \toprule
    \multirow{2}{*}{\textbf{Method}} &
    \multicolumn{7}{c}{Abs.Rel.$\downarrow$} \\
    \cmidrule{2-8}
    & \textit{Front}
    & \textit{F.Left}
    & \textit{F.Right}
    & \textit{B.Left}
    & \textit{B.Right}
    & \textit{Back}
    & \textit{Avg.}
    \\
    \midrule
    Mono$^\dagger$ - M
    & 0.184
    & 0.366
    & 0.448
    & 0.417
    & 0.426
    & 0.438
    & 0.380
    \\
    Mono$^\dagger$
    & 0.139
    & 0.209
    & 0.236
    & 0.231
    & 0.247
    & 0.204
    & 0.211
    \\
    \textbf{FSM$^\dagger$}
    & \underline{0.131}
    & \underline{0.203}
    & \underline{0.226}
    & \textbf{0.223}
    & \textbf{0.240}
    & \underline{0.188}
    & \underline{0.202}
    \\
    \midrule
    Mono$^\ddagger$
    & 0.143
    & 0.238
    & 0.265
    & 0.277
    & 0.276
    & 0.247
    & 0.241
    \\
    \textbf{FSM$^\ddagger$}
    & 0.133
    & 0.212
    & 0.229
    & 0.231
    & \underline{0.246}
    & 0.194
    & 0.208
    \\ 
    \midrule
    \textbf{FSM - STC}
    & 0.133
    & 0.219
    & 0.246
    & 0.252
    & 0.259
    & 0.197
    & 0.218
    \\
    \textbf{FSM - PCC}
    & \underline{0.131}
    & 0.206
    & 0.228
    & 0.238 
    & 0.248
    & \underline{0.188}
    & 0.207
    \\
    \textbf{FSM}
    & \textbf{0.130}
    & \textbf{0.201}
    & \textbf{0.224}
    & \underline{0.229}
    & \textbf{0.240}
    & \textbf{0.186}
    & \textbf{0.201}
    \\
    \bottomrule
\end{tabular}
}
\\
\vspace{-2mm}
\subfloat[nuScenes]{
\begin{tabular}{l|cccccc|c}
    \toprule
    \multirow{2}{*}{\textbf{Method}} &
    \multicolumn{6}{c}{Abs.Rel.$\downarrow$} \\
    \cmidrule{2-8}
    & \textit{Front}
    & \textit{F.Left}
    & \textit{F.Right}
    & \textit{B.Left}
    & \textit{B.Right}
    & \textit{Back}
    & \textit{Avg.}
    \\
    \midrule
    Mono(PP\_GT)
    & 0.214
    & 0.304
    & 0.388
    & 0.314 
    & 0.438 
    & 0.304 
    & 0.327 
    \\
    FSM(PP\_GT)
    & 0.198
    & 0.297
    & 0.364
    & \underline{0.301} 
    & 0.392
    & \underline{0.240}
    & \underline{0.299}
    \\
    \midrule
    Mono(Shared)
    & 0.251
    & 0.403 
    & 0.546
    & 0.429 
    & 0.616 
    & 0.321 
    & 0.428
    \\
    FSM(Shared))
    & 0.200 
    & 0.337 
    & 0.448
    & 0.354 
    & 0.521 
    & 0.267 
    & 0.355 
    \\ 
    \midrule
    Mono (PP\_GT) % modified
    & \textbf{0.204}
    & 0.332 
    & \textbf{0.380}
    & 0.323 
    & \textbf{0.407} 
    & \textbf{0.223} 
    & \textbf{0.312}
    \\
    Mono (PP) % modified
    & 0.209 
    & 0.405 
    & 0.461
    & 0.457 
    & 0.518 
    & 0.233 
    & 0.381
    % \\ 
    % \textbf{FSM}
    % & \textbf{0.186}
    % & \textbf{0.287}
    % & \underline{0.375}
    % & \textbf{0.296}
    % & \underline{0.418}
    % & \textbf{0.221}
    % & \textbf{0.297}
    \\
    \bottomrule
\end{tabular}
}
% \vspace{-2mm}
\caption{\textbf{Depth estimation results on multi-camera datasets}, using \emph{FSM} relative to the single-camera photometric loss (\emph{Mono}). The symbol $^\dagger$ denotes per-frame median-scaling, and $^\ddagger$ shared median-scaling (Eq.~\ref{eq:sharedmedscaling}). \emph{M} denotes the removal of masking (Sec.~\ref{sec:mask}), \emph{STC} the removal of spatio-temporal contexts (Sec.~\ref{sec:stc}), and \emph{PCC} the removal of pose consistency constraints (Sec.~\ref{sec:pcc}).}
\label{tab:both_scaling_small}
% \vspace{-3mm}
\end{table}

==> tables/ddad_6camera.tex <==

\begin{table}%
    % \vspace{-1mm}
    \centering
    \small
    \renewcommand{\arraystretch}{1.00}
    \setlength{\tabcolsep}{0.22em}
    \subfloat[With median scaling]{
    \begin{tabular}{l|cccccc|c}
        \toprule
        \multirow{2}{*}{\textbf{Model}} &
        \multicolumn{7}{c}{Abs.Rel.$\downarrow$ (Median)} \\
        \cmidrule{2-8}
        & \textit{Front}
        & \textit{F.Left}
        & \textit{F.Right}
        & \textit{B.Left}
        & \textit{B.Right}
        & \textit{Back}
        & \textit{Avg.}
        \\
        \midrule
        Mono-Pre % glorious-grass-13154, e=15
        & 0.163
        & 0.202
        & 0.232
        & 0.231
        & 0.247
        & 0.214
        & 0.215 % 0.2148
        \\
        \midrule
        \textbf{Self-FSM} % ANOVA, 
        & 0.158
        & \textbf{0.200}
        & \textbf{0.224} 
        & \textbf{0.217}
        & \textbf{0.233}
        & 0.216
        & 0.208
        \\
        (S.D.) % ANOVA, 
        & .001
        & .001
        & .001
        & .001
        & .001
        & .001
        & .025
        \\
        \midrule
        Mono\textasteriskcentered % ANOVA
        & 0.160
        & 0.201
        & 0.227
        & \textbf{0.217}
        & 0.234
        & 0.218
        & 0.210
        \\
        (S.D.) % ANOVA
        & .001
        & .001
        & .001
        & .002
        & .001
        & .001
        & .025
        \\
        \midrule
        FSM\textasteriskcentered % valiant-wind-13166, e=5
        & 0.158
        & 0.200
        & 0.226
        & 0.218
        & 0.234
        & 0.216
        & 0.209
        \\
        (S.D.) % peachy-sun-13162, e=5
        & .001
        & .001
        & .001
        & .002
        & .002
        & .001
        & .025
        \\
        \midrule
        \midrule
        % Mono~\cite{packnet}
        % & 0.139
        % & 0.209
        % & 0.236
        % & 0.231
        % & 0.247
        % & 0.204
        % & 0.211
        % \\
        FSM~\cite{fsm20222}
        & \textbf{0.131}
        & 0.203
        & 0.226
        & 0.223
        & 0.240
        & \textbf{0.188}
        & \textbf{0.202}
        \\
        \bottomrule
    \end{tabular}
    }
    \\
    \vspace{-2mm}
    \subfloat[Without median scaling]{
    \begin{tabular}{l|cccccc|c}
        \toprule
        \multirow{2}{*}{\textbf{Model}} &
        \multicolumn{7}{c}{Abs.Rel.$\downarrow$ (Metric)} \\
        \cmidrule{2-8}
        & \textit{Front}
        & \textit{F.Left}
        & \textit{F.Right}
        & \textit{B.Left}
        & \textit{B.Right}
        & \textit{Back}
        & \textit{Avg.}
        \\
        \midrule
        Mono-Pre % glorious-grass-13154
        & 0.169
        & 0.203
        & 0.228
        & 0.235
        & 0.238
        & 0.206
        & 0.213 % .2131
        \\
        \midrule
        \textbf{Self-FSM} % ANOVA
        & 0.161
        & \textbf{0.195}
        & \textbf{0.216}
        & \textbf{0.215}
        & \textbf{0.221}
        & 0.207
        & \underline{0.202}
        \\
        (S.D.) % peachy-sun-13162, e=5
        & .001
        & .001
        & .001
        & .002
        & .001
        & .001
        & .020
        \\
        \midrule
        Mono\textasteriskcentered % peachy-sun-13162, e=5
        & 0.165
        & 0.196
        & 0.219
        & 0.216
        & 0.222
        & 0.209
        & 0.205
        \\
        (S.D.) % peachy-sun-13162, e=5
        & .001
        & .000
        & .001
        & .002
        & .001
        & .002
        & .020
        \\
        \midrule
        FSM\textasteriskcentered % valiant-wind-13166, e=5
        & 0.162
        & 0.196
        & 0.217
        & 0.216
        & 0.222
        & 0.206
        & 0.203
        \\
        (S.D.) % peachy-sun-13162, e=5
        & .001
        & .002
        & .002
        & .003
        & .003
        & .002
        & .020
        \\
        \midrule
        \midrule
        % Mono~\cite{packnet}
        % & -
        % & -
        % & -
        % & -
        % & -
        % & -
        % & -
        % \\
        FSM~\cite{fsm20222}
        & \textbf{0.130}
        & 0.201
        & 0.224
        & 0.229
        & 0.240
        & \textbf{0.186}
        & \textbf{0.201}
        \\
        \bottomrule
    \end{tabular}
    }
    % \vspace{-2mm}
    \caption{\textbf{Depth estimation results by ResNet18-based model on DDAD}. 
    Starting from the scale-aware pretrained monodepth model (\emph{Mono-Pre}), the model with predicted extrinsics (\emph{Self-FSM}), the baseline model (\emph{Mono\textasteriskcentered}), and the model which can use ground truth extrinsics (\emph{FSM}) are finetuned. The symbol \textasteriskcentered denotes our implementation. (S.D.) is the standard deviation calculated by $n=7$ for each camera, and $n=42$ for averaged performance through the method (described in \textit{Avg.}).}
    \label{tab:depth_ddad}
    \end{table}
    

==> tables/ddad_ablation.tex <==

\captionsetup[table]{skip=6pt}

\begin{table}[t!]
\vspace{-3mm}
\renewcommand{\arraystretch}{0.9}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|c|cccc}
\toprule
\textbf{Method} & \textbf{Sup.} & 
Abs Rel$\downarrow$ &
Sq Rel$\downarrow$ &
RMSE$\downarrow$ &
$\delta_{1.25}$ $\uparrow$
\\
\toprule
SuperDepth~\cite{superdepth} 
& $S$ & 0.112 & 0.875 & 4.958 & 0.852 \\
Monodepth2~\cite{godard2019digging} 
& $M$ & 0.115 & 0.903 & 4.863 & 0.877 \\
Monodepth2~\cite{godard2019digging} 
& $S$ & 0.109 & 0.873 & 4.960 & 0.864 \\
\midrule
Monodepth2~\cite{godard2019digging} 
& $M+S$ & \textbf{0.106} & \textbf{0.818} & 4.750 & \textbf{0.874} \\
Ours & $STC$ & 0.112 & 0.767 & \textbf{4.705} & 0.864 \\
\bottomrule
\end{tabular}
}
\caption{
\textbf{Ablation experiments on DDAD}, to validate the various components and design choices of our proposed architecture.}
\label{table:ddad_ablation}
\vspace{-3mm}
\end{table}

==> tables/ddad_depth.tex <==
\captionsetup[table]{skip=6pt}

\begin{table}[t!]
% \vspace{-3mm}
%\vspace{-4mm}
%\rowcolors{2}{lightgray}{white}
\renewcommand{\arraystretch}{1.00}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|cccc}
\toprule
\textbf{Method}  & 
Abs Rel$\downarrow$ &
Sq Rel$\downarrow$ &
RMSE$\downarrow$ &
$\delta_{1.25}$ $\uparrow$
\\
\toprule
COLMAP (pseudo-depth) & 
0.243 & 4.438 & 17.239 & 0.601 \\
\midrule
Monodepth2$^\dagger$ (R18)~\cite{godard2019digging}  &
0.213 & 4.975 & 18.051 & 0.761 \\
Monodepth2$^\dagger$ (R50)~\cite{godard2019digging} &
0.198 & 4.504 & 16.641 & 0.781 \\
PackNet$^\dagger$~\cite{packnet}  &
0.162 & 3.917 & \textbf{13.452} & 0.823 \\
\midrule
\textbf{FSM}$^\dagger$ (w/o mask \& spatial) & 0.184 & 4.049 & 17.109 & 0.735 \\
\textbf{FSM}$^\dagger$ (w/o spatial) & 0.139 & 3.023 & 14.106 & 0.827 \\
\textbf{FSM} (w/ spatial) & 0.135 & 2.841 & 13.850 & 0.832 \\
\textbf{FSM} (w/ spatio-temporal) & \textbf{0.130} & \textbf{2.731} & 13.654 & \textbf{0.837} \\

\bottomrule
\end{tabular}
}
\caption{
\textbf{Quantitative depth evaluation of different methods on the DDAD \cite{packnet} dataset}, for distances up to 200m on the forward-facing camera. The symbol $\dagger$ denotes per-frame median scaling.
}
% \vspace{-6mm}
\label{table:ddad_depth}
\end{table}

==> tables/ddad_scaling.tex <==

\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{1.0}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|c|cccccc|cccccc}
\toprule
\multirow{2}{*}{\rotatebox{45}{\textbf{Method}}} &
\multirow{2}{*}{\rotatebox{45}{\textbf{Scaling}}} &
\multicolumn{6}{c}{Abs.Rel.$\downarrow$} &
\multicolumn{6}{|c}{$\delta < 1.25\uparrow$} \\
\cmidrule{3-14}
& 
& \textit{Front}
& \textit{F.Left}
& \textit{F.Right}
& \textit{B.Left}
& \textit{B.Right}
& \textit{Back}
& \textit{Front}
& \textit{F.Left}
& \textit{F.Right}
& \textit{B.Left}
& \textit{B.Right}
& \textit{Back}
\\
\midrule
Mono
& Indiv. 
& 0.139
& 0.209
& 0.236
& 0.231
& 0.247
& 0.204
& 0.832
& 0.709
& 0.673
& 0.686
& 0.660
& 0.695
\\
\textbf{MultiCam}
& Indiv.
& 0.131
& 0.203
& 0.226
& 0.223
& 0.240
& 0.188
& 0.840
& 0.716
& 0.687
& 0.693
& 0.670
& 0.714
\\
\midrule
Mono
& Shared
& 0.143
& 0.227
& 0.253
& 0.264
& 0.263
& 0.236
& 0.828
& 0.623
& 0.582
& 0.509
& 0.530
& 0.558
\\
\textbf{MultiCam}
& Shared
& 0.133
& 0.212
& 0.239
& 0.241
& 0.256
& 0.194
& 0.837
& 0.673
& 0.639
& 0.600
& 0.585
& 0.683
\\ 
\midrule
\textbf{MultiCam - STC}
& ---
& 0.133
& 0.219
& 0.246
& 0.252
& 0.259
& 0.197
& 0.830
& 0.627
& 0.599
& 0.552
& 0.554
& 0.674
\\
\textbf{MultiCam}
& ---
& 0.131
& 0.206
& 0.228
& 0.238 
& 0.248
& 0.188
& 0.831
& 0.669
& 0.650
& 0.594
& 0.587
& 0.687
\\
\bottomrule

% \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textit{Mono (Standard)}}}} 
% & 01 & 0.139 & 3.023 & 13.835 & 0.234 & 22.782 & 0.832 & 0.937 & 0.970
% \\
% & 05 & 0.209 & 3.410 & 12.609 & 0.319 & 30.722 & 0.709 & 0.881 & 0.938
% \\
% & 06 & 0.236 & 3.827 & 12.097 & 0.344 & 33.294 & 0.673 & 0.860 & 0.928
% \\
% & 07 & 0.231 & 3.976 & 12.311 & 0.331 & 31.874 & 0.686 & 0.863 & 0.931
% \\
% & 08 & 0.247 & 3.776 & 11.449 & 0.354 & 33.996 & 0.660 & 0.850 & 0.925
% \\
% & 09 & 0.204 & 3.345 & 14.371 & 0.309 & 30.150 & 0.695 & 0.889 & 0.949
% \\

% \midrule

% \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textit{Mono (Shared)}}}} 
% & 01 & 0.143 & 3.133 & 13.875 & 0.237 & 23.029 & 0.828 & 0.935 & 0.970
% \\
% & 05 & 0.227 & 3.624 & 13.545 & 0.365 & 30.685 & 0.623 & 0.840 & 0.917
% \\
% & 06 & 0.253 & 4.197 & 13.324 & 0.400 & 33.375 & 0.582 & 0.821 & 0.905
% \\
% & 07 & 0.264 & 4.103 & 14.038 & 0.419 & 31.827 & 0.509 & 0.778 & 0.890
% \\
% & 08 & 0.263 & 3.856 & 12.739 & 0.419 & 34.001 & 0.530 & 0.795 & 0.896
% \\
% & 09 & 0.236 & 4.235 & 16.729 & 0.386 & 30.137 & 0.558 & 0.814 & 0.911
% \\

% \midrule
% \midrule

% \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textit{Multi (Standard)}}}} 
% & 01 & 0.135 & 2.841 & 13.850 & 0.230 & 23.378 & 0.832 & 0.939 & 0.972
% \\
% & 05 & 0.207 & 3.239 & 12.608 & 0.320 & 30.793 & 0.705 & 0.879 & 0.938
% \\
% & 06 & 0.231 & 3.648 & 11.928 & 0.341 & 33.092 & 0.676 & 0.862 & 0.931
% \\
% & 07 & 0.225 & 3.804 & 12.341 & 0.330 & 31.804 & 0.688 & 0.863 & 0.930
% \\
% & 08 & 0.240 & 3.525 & 11.277 & 0.350 & 33.776 & 0.667 & 0.854 & 0.928
% \\
% & 09 & 0.200 & 3.379 & 14.934 & 0.312 & 30.450 & 0.694 & 0.887 & 0.948
% \\

% \midrule

% \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textit{Multi (Shared)}}}} 
% & 01 & 0.138 & 2.924 & 14.041 & 0.232 & 22.557 & 0.826 & 0.937 & 0.971
% \\
% & 05 & 0.218 & 3.363 & 13.172 & 0.351 & 30.966 & 0.655 & 0.848 & 0.923
% \\
% & 06 & 0.241 & 3.896 & 12.827 & 0.377 & 32.893 & 0.621 & 0.835 & 0.914
% \\
% & 07 & 0.249 & 3.761 & 13.289 & 0.384 & 32.133 & 0.580 & 0.818 & 0.908
% \\
% & 08 & 0.257 & 3.549 & 12.096 & 0.393 & 33.719 & 0.568 & 0.821 & 0.910
% \\
% & 09 & 0.205 & 3.629 & 15.419 & 0.334 & 30.211 & 0.668 & 0.865 & 0.936
% \\

% \midrule
% \midrule

% \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textit{Multi (Aware)}}}} 
% & 01 & 0.137 & 3.027 & 14.220 & 0.237 & 22.596 & 0.821 & 0.934 & 0.970
% \\
% & 05 & 0.211 & 3.335 & 13.219 & 0.350 & 30.966 & 0.661 & 0.849 & 0.923
% \\
% & 06 & 0.231 & 3.844 & 12.860 & 0.375 & 32.893 & 0.639 & 0.835 & 0.912
% \\
% & 07 & 0.244 & 3.731 & 13.303 & 0.384 & 32.133 & 0.589 & 0.814 & 0.907
% \\
% & 08 & 0.247 & 3.512 & 12.140 & 0.390 & 33.719 & 0.584 & 0.824 & 0.910
% \\
% & 09 & 0.191 & 3.479 & 15.370 & 0.328 & 30.211 & 0.693 & 0.869 & 0.937
% \\

\bottomrule

\end{tabular}
}
\caption{\textbf{Depth estimation results on DDAD}, using our proposed spatio-temporal photometric loss (\textit{Multi}) relative to the standard photometric loss (\textit{Mono}). The \textit{Standard} evaluation uses per-frame ground truth median scaling at test time; the \textit{Shared} evaluation uses our proposed per-sample ground-truth median scaling, using all six cameras; and the \textit{Aware} evaluation does not use median scaling at test time. Using the standard median scaling evaluation, our results are on-par with, our } 
\label{tab:depth_ddad}
\end{table*}





==> tables/ddad_scaling_small.tex <==

\begin{table}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{1.0}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|c|cccccc}
\toprule
\multirow{2}{*}{} &
\multirow{2}{*}{\rotatebox{90}{\textbf{Scaling}}} &
\multicolumn{6}{c}{Abs.Rel.$\downarrow$} \\
\cmidrule{3-8}
& 
& \textit{Front}
& \textit{F.Left}
& \textit{F.Right}
& \textit{B.Left}
& \textit{B.Right}
& \textit{Back}
\\
\midrule
Mono $-$ M
& F
& 0.184
& 0.366
& 0.448
& 0.417
& 0.426
& 0.438
\\
Mono
& F 
& 0.139
& 0.209
& 0.236
& 0.231
& 0.247
& 0.204
\\
\textbf{FSM}
& F
& \underline{0.131}
& \underline{0.203}
& \underline{0.226}
& \textbf{0.223}
& \textbf{0.240}
& \underline{0.188}
\\
\midrule
Mono
& S
& 0.143
& 0.238
& 0.265
& 0.277
& 0.276
& 0.247
\\
\textbf{FSM}
& S
& 0.133
& 0.212
& 0.229
& 0.231
& 0.246
& 0.194
\\ 
\midrule
\textbf{FSM $-$ STC}
& -
& 0.133
& 0.219
& \underline{0.246}
& 0.252
& 0.259
& 0.197
\\
\textbf{FSM $-$ PCC}
& -
& \underline{0.131}
& 0.206
& 0.228
& 0.238 
& 0.248
& \underline{0.188}
\\
\textbf{FSM}
& -
& \textbf{0.130}
& \textbf{0.201}
& \textbf{0.224}
& \underline{0.229}
& \textbf{0.240}
& \textbf{0.186}
\\
\bottomrule
\end{tabular}
}
\caption{\textbf{Depth estimation results on DDAD}, using our proposed \emph{FSM} approach relative to the standard single-camera photometric loss (\emph{Mono}). In the scaling column, \emph{I} denotes per-frame median scaling, and \emph{S} our proposed shared median scaling.}
\label{tab:depth_ddad_small}
\end{table}





==> tables/many_colmap.tex <==
%Extrinsics Evaluation
\begin{table}%
% \vspace{-1mm}
\centering
\small
\renewcommand{\arraystretch}{1.00}
\setlength{\tabcolsep}{0.22em}
\subfloat[Translation error (Euclidean) \lbrack m\rbrack]{
\begin{tabular}{l|ccc}
    \toprule
    \multirow{2}{*}{\textbf{Method}} &
    \multicolumn{3}{c}{$t\ [m] \downarrow$ (Mean $\pm$ S.D.)} \\
    \cmidrule{2-4}
    & \emph{seq}:000052
    & \emph{seq}:000033
    & \emph{seq}:000016
    \\
    \midrule
    COLMAP % (.105+.102+.104+.113+.066)/5
    & 0.098$\pm$0.017
    & 0.164$\pm$0.080
    & 0.797$\pm$0.384
    \\
    \textbf{Self-FSM} % (0.050+0.051+0.074+0.062+0.071)/5
    & \textbf{0.062$\pm$0.010}
    & \textbf{0.073$\pm$0.036}
    & \textbf{0.174$\pm$0.103}
    \\
    \bottomrule
\end{tabular}
}
\\
\vspace{-2mm}
\subfloat[Translaiton error (Cosine similarity)]{
    \begin{tabular}{l|ccc}
        \toprule
        \multirow{2}{*}{\textbf{Method}} &
        \multicolumn{3}{c}{$t\ [^{\circ}]\downarrow$ (Mean $\pm$ S.D.)} \\
        \cmidrule{2-4}
        & \emph{seq}:000052
        & \emph{seq}:000033
        & \emph{seq}:000016
        \\
        \midrule
        COLMAP % (.105+.102+.104+.113+.066)/5
        & 10.8$\pm$11.0
        & 13.2$\pm$6.25
        & 44.2$\pm$17.4
        \\
        \textbf{Self-FSM} % (0.050+0.051+0.074+0.062+0.071)/5
        & \textbf{5.89$\pm$3.70}
        & \textbf{5.02$\pm$5.13}
        & \textbf{9.61$\pm$4.76}
        \\
        \bottomrule
    \end{tabular}
}
\\
\vspace{-2mm}
\subfloat[Rotation error (Geodesic)]{
    \begin{tabular}{l|ccc}
        \toprule
        \multirow{2}{*}{\textbf{Method}} &
        \multicolumn{3}{c}{$t\ [^{\circ}]\downarrow$ (Mean $\pm$ S.D.)} \\
        \cmidrule{2-4}
        & \emph{seq}:000052
        & \emph{seq}:000033
        & \emph{seq}:000016
        \\
        \midrule
        COLMAP % (.105+.102+.104+.113+.066)/5
        & 0.540$\pm$0.269
        & 0.655$\pm$0.281
        & 2.23$\pm$1.23
        \\
        \textbf{Self-FSM} % (0.050+0.051+0.074+0.062+0.071)/5
        & \textbf{0.190$\pm$0.043}
        & \textbf{0.429$\pm$0.064}
        & \textbf{0.296$\pm$0.175}
        \\
        \bottomrule
    \end{tabular}
}
% \vspace{-2mm}
\caption{\textbf{Quantitative result of the calibration result on DDAD.}. The error is represented as the mean and standard deviation of the five cameras in each sequence. 
}
\label{tab:many_colmap}
% \vspace{-3mm}
\end{table}

==> tables/nuscenes_scaling.tex <==

\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{1.0}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|c|cccccc|cccccc}
\toprule
\multirow{2}{*}{\rotatebox{45}{\textbf{Method}}} &
\multirow{2}{*}{\rotatebox{45}{\textbf{Scaling}}} &
\multicolumn{6}{c}{Abs.Rel.$\downarrow$} &
\multicolumn{6}{|c}{$\delta < 1.25\uparrow$} \\
\cmidrule{3-14}
& 
& \textit{Front}
& \textit{F.Left}
& \textit{B.Left}
& \textit{Back}
& \textit{B.Right}
& \textit{F.Right}
& \textit{Front}
& \textit{F.Left}
& \textit{B.Left}
& \textit{Back}
& \textit{B.Right}
& \textit{F.Right}
\\
\midrule
Mono
& Indiv. 
& 0.248
& 0.315
& 0.304 
& 0.304 
& 0.417 
& 0.398
& 0.727
& 0.629
& 0.659
& 0.712 
& 0.594
& 0.603
\\
\textbf{MultiCam}
& Indiv.
& 0.198
& 0.297
& 0.289 
& 0.240
& 0.392
& 0.350
& 0.748
& 0.643
& 0.670
& 0.731
& 0.620
& 0.631
\\
\midrule
Mono
& Shared
& 0.251
& 0.403 
& 0.429 
& 0.321 
& 0.616 
& 0.546
& 0.729
& 0.520
& 0.511
& 0.659 
& 0.497
& 0.508
\\
\textbf{MultiCam}
& Shared
& 0.200 
& 0.337 
& 0.354 
& 0.267 
& 0.521 
& 0.448
& 0.754
& 0.574
& 0.567
& 0.687 
& 0.549
& 0.558
\\ 
\midrule
\textbf{MultiCam - STC}
& ---
& 0.208
& 0.382
& 0.393
& 0.258
& 0.595
& 0.510
& 0.691
& 0.526
& 0.516
& 0.680
& 0.536
& 0.542
\\ 
\textbf{MultiCam}
& ---
& 0.187 
& 0.291
& 0.311
& 0.235
& 0.448
& 0.392
& 0.736
& 0.602
& 0.576
& 0.710
& 0.592
& 0.606
\\
\bottomrule


\bottomrule

\end{tabular}
}
\caption{\textbf{Depth estimation results on nuScenes}, using our proposed spatio-temporal photometric loss (\textit{Multi} relative to the standard photometric loss (\textit{Mono}). The \textit{Standard} evaluation uses per-frame ground truth median scaling at test time; the \textit{Shared} evaluation uses our proposed per-sample ground-truth median scaling, using all six cameras; and the \textit{Aware} evaluation does not use median scaling at test time. Using the standard median scaling evaluation, our results are on-par with, our } 
\label{tab:depth_nuscenes}
\end{table*}





==> tables/nuscenes_scaling_small.tex <==

\begin{table}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{1.0}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|c|cccccc}
\toprule
\multirow{2}{*}{} &
\multirow{2}{*}{\rotatebox{90}{\textbf{Scaling}}} &
\multicolumn{6}{c}{Abs.Rel.$\downarrow$} \\
\cmidrule{3-8}
& 
& \textit{Front}
& \textit{F.Left}
& \textit{B.Left}
& \textit{Back}
& \textit{B.Right}
& \textit{F.Right}
\\
\midrule
Mono
& F 
& 0.214
& 0.304
& 0.294 
& 0.304 
& 0.408 
& 0.368
\\
\textbf{FSM}
& F
& 0.198
& 0.297
& 0.289 
& 0.240
& 0.392
& 0.350
\\
\midrule
Mono
& S
& 0.251
& 0.403 
& 0.429 
& 0.321 
& 0.616 
& 0.546
\\
\textbf{FSM}
& S
& 0.200 
& 0.337 
& 0.354 
& 0.267 
& 0.521 
& 0.448
\\ 
\midrule
\textbf{FSM $-$ STC}
& -
& 0.208
& 0.382
& 0.393
& 0.258
& 0.595
& 0.510
\\ 
\textbf{FSM $-$ PCC}
& -
& 0.187 
& 0.291
& 0.311
& 0.235
& 0.448
& 0.392
\\ 
\textbf{FSM}
& -
& \textbf{0.186}
& \textbf{0.287}
& 0.296
& 0.221
& 0.418
& 0.375
\\
\bottomrule

\end{tabular}
}
\caption{\textbf{Depth estimation results on nuScenes}, using FSM relative to the standard single-camera photometric loss. In the scaling column, \emph{I} denotes per-frame median scaling, and \emph{S} our proposed shared median scaling. \emph{M} refers to the removal of self-occlusion masks, and \emph{STC} to the removal of spatio-temporal constraints.}
\label{tab:depth_nuscenes_small}
\end{table}





==> tables/nuscenes_tmp.tex <==

\begin{table*}[t!]
    %\vspace{-4mm}
    \renewcommand{\arraystretch}{1.0}
    \centering
    {
    \small
    \setlength{\tabcolsep}{0.3em}
    \begin{tabular}{l|c|cccccc|cccccc}
    \toprule
    \multirow{2}{*}{\rotatebox{45}{\textbf{Method}}} &
    \multirow{2}{*}{\rotatebox{45}{\textbf{Scaling}}} &
    \multicolumn{6}{c}{Abs.Rel.$\downarrow$} &
    \multicolumn{6}{|c}{$\delta < 1.25\uparrow$} \\
    \cmidrule{3-14}
    & 
    & \textit{Front}
    & \textit{F.Left}
    & \textit{B.Left}
    & \textit{Back}
    & \textit{B.Right}
    & \textit{F.Right}
    & \textit{Front}
    & \textit{F.Left}
    & \textit{B.Left}
    & \textit{Back}
    & \textit{B.Right}
    & \textit{F.Right}
    \\
    \midrule
    Mono
    & Indiv. 
    & 0.248
    & 0.315
    & 0.304 
    & 0.304 
    & 0.417 
    & 0.398
    & 0.727
    & 0.629
    & 0.659
    & 0.712 
    & 0.594
    & 0.603
    \\
    \textbf{MultiCam}
    & Indiv.
    & 0.198
    & 0.297
    & 0.289 
    & 0.240
    & 0.392
    & 0.350
    & 0.748
    & 0.643
    & 0.670
    & 0.731
    & 0.620
    & 0.631
    \\
    \midrule
    Mono
    & Shared
    & 0.251
    & 0.403 
    & 0.429 
    & 0.321 
    & 0.616 
    & 0.546
    & 0.729
    & 0.520
    & 0.511
    & 0.659 
    & 0.497
    & 0.508
    \\
    \textbf{MultiCam}
    & Shared
    & 0.200 
    & 0.337 
    & 0.354 
    & 0.267 
    & 0.521 
    & 0.448
    & 0.754
    & 0.574
    & 0.567
    & 0.687 
    & 0.549
    & 0.558
    \\ 
    \midrule
    \textbf{MultiCam - STC}
    & ---
    & 0.208
    & 0.382
    & 0.393
    & 0.258
    & 0.595
    & 0.510
    & 0.691
    & 0.526
    & 0.516
    & 0.680
    & 0.536
    & 0.542
    \\ 
    \textbf{MultiCam}
    & ---
    & 0.187 
    & 0.291
    & 0.311
    & 0.235
    & 0.448
    & 0.392
    & 0.736
    & 0.602
    & 0.576
    & 0.710
    & 0.592
    & 0.606
    \\
    \bottomrule
    
    
    \bottomrule
    
    \end{tabular}
    }
    \caption{\textbf{Depth estimation results on nuScenes}, using our proposed spatio-temporal photometric loss (\textit{Multi} relative to the standard photometric loss (\textit{Mono}). The \textit{Standard} evaluation uses per-frame ground truth median scaling at test time; the \textit{Shared} evaluation uses our proposed per-sample ground-truth median scaling, using all six cameras; and the \textit{Aware} evaluation does not use median scaling at test time. Using the standard median scaling evaluation, our results are on-par with, our } 
    \label{tab:depth_nuscenes}
    \end{table*}
    
    
    
    

==> tables/suppmat_networks.tex <==
\begin{table}[t!]%
\small
  \centering
\resizebox{0.84\linewidth}{!}{
\subfloat[][Depth Network \cite{monodepth2}.]{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[b]{l|l|c|c|c}
\toprule
& \textbf{Layer Description} & \textbf{K} & \textbf{S} & \textbf{Out. Dim.} \\ 
\toprule
\multicolumn{5}{c}{\textbf{ResidualBlock (K, S)}} \\ 
\midrule
\#A & Conv2d $\shortrightarrow$ BN $\shortrightarrow$ ReLU & K & 1 &  \\
\#B & Conv2d $\shortrightarrow$ BN $\shortrightarrow$ ReLU & K & S &  \\
\toprule
\multicolumn{5}{c}{\textbf{UpsampleBlock (\#skip)}} \\ 
\midrule
\#C & Conv2d $\shortrightarrow$ BN $\shortrightarrow$ ReLU $\shortrightarrow$ Upsample         & 3 & 1 & \\
\#D & Conv2d ($\#C \oplus \#skip$) $\shortrightarrow$ BN $\shortrightarrow$ ReLU  & 3 & 1 & \\
\toprule
\toprule
\#0 & Input RGB image & - & - & 3$\times$H$\times$W \\ 
\midrule
\multicolumn{5}{c}{\textbf{Encoder}} \\ \hline
\#1  & Conv2d $\shortrightarrow$ BN $\shortrightarrow$ ReLU   & 7 & 1 &  64$\times$H$\times$W \\
\#2  & Max. Pooling                 & 3 & 2 &  64$\times$H/2$\times$W/2 \\
\#3  & ResidualBlock (x2)           & 3 & 2 &  64$\times$H/4$\times$W/4 \\
\#4  & ResidualBlock (x2)           & 3 & 2 & 128$\times$H/8$\times$W/8 \\
\#5  & ResidualBlock (x2)           & 3 & 2 & 256$\times$H/16$\times$W/16 \\
\#6  & ResidualBlock (x2)           & 3 & 2 & 512$\times$H/32$\times$W/32 \\
\midrule
\multicolumn{5}{c}{\textbf{Depth Decoder}} \\ 
\midrule
\#7 & UpsampleBlock (\#5)    & 3 & 1 & 256$\times$H/16$\times$W/16 \\
\#8 & UpsampleBlock (\#4)    & 3 & 1 & 128$\times$H/8$\times$W/8 \\
\#9 & UpsampleBlock (\#3)    & 3 & 1 & 64$\times$H/4$\times$W/4 \\
\#10 & UpsampleBlock (\#2)   & 3 & 1 & 32$\times$H/2$\times$W/2 \\
\#11 & UpsampleBlock (\#1)   & 3 & 1 & 32$\times$H$\times$W \\
\#12 & Conv2d $\shortrightarrow$ Sigmoid  & 3 & 1 & 1$\times$H$\times$W \\
\bottomrule
\end{tabular}
\label{tab:netdepth}
}}
\\
\resizebox{0.84\linewidth}{!}{
\subfloat[][Pose Network \cite{zhou2018unsupervised}.]{
\begin{tabular}[b]{l|c|c|c|c}
\toprule
& \textbf{Layer Description} & \textbf{K} & \textbf{S} & \textbf{Out. Dim.} \\ 
\toprule
\#0 & Input 2 RGB images & - & - & 6$\times$H$\times$W \\ 
\midrule
\#1  & \hspace{2mm} Conv2d $\shortrightarrow$ GN $\shortrightarrow$ ReLU \hspace{2mm} & 3 & 2 & 16$\times$H/2$\times$W/2 \\
\#2  & \hspace{2mm} Conv2d $\shortrightarrow$ GN $\shortrightarrow$ ReLU \hspace{2mm} & 3 & 2 & 32$\times$H/4$\times$W/4 \\
\#3  & \hspace{2mm} Conv2d $\shortrightarrow$ GN $\shortrightarrow$ ReLU \hspace{2mm} & 3 & 2 & 64$\times$H/8$\times$W/8 \\
\#4  & \hspace{2mm} Conv2d $\shortrightarrow$ GN $\shortrightarrow$ ReLU \hspace{2mm} & 3 & 2 & 128$\times$H/16$\times$W/16 \\
\#5  & \hspace{2mm} Conv2d $\shortrightarrow$ GN $\shortrightarrow$ ReLU \hspace{2mm} & 3 & 2 & 256$\times$H/32$\times$W/32 \\
\#6  & \hspace{2mm} Conv2d $\shortrightarrow$ GN $\shortrightarrow$ ReLU \hspace{2mm} & 3 & 2 & 256$\times$H/64$\times$W/64 \\
\#7  & \hspace{2mm} Conv2d $\shortrightarrow$ GN $\shortrightarrow$ ReLU \hspace{2mm} & 3 & 2 & 256$\times$H/128$\times$W/128 \\
\#8  & Conv2d & 1 & 1 & 6$\times$H/128$\times$W/128 \\
\midrule
\#9  & Global Pooling & - & - & 6 \\
\bottomrule
\end{tabular}
\label{tab:netpose}
}}
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{
\textbf{Neural network architectures used in our proposed FSM framework}. The predicted depth maps are $1 \times H \times W$ tensors, and the predicted poses are $6$-dimensional vectors representing translation ($x,y,z$) and Euler rotation angles (pitch, yaw, roll).  \emph{BN} stands for Batch Normalization \cite{ioffe2015batch}, \emph{GN} for Group Normalization \cite{WuH18}, \emph{Upsample} doubles spatial dimensions using bilinear interpolation, and \emph{ReLU} denote Rectified Linear Units. The symbol $\oplus$ indicates feature concatenation. 
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{tab:networks}
\vspace{-5mm}
\end{table}


==> tables/table_metric_ddad.tex <==
\captionsetup[table]{skip=6pt}

\begin{table}[t!]
% \vspace{-4mm}
\renewcommand{\arraystretch}{1.00}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|cccccc|c}
    \toprule
    \multirow{2}{*}{\textbf{Model}} &
    \multicolumn{7}{c}{Abs.Rel.$\downarrow$ (Metric)} \\
    \cmidrule{2-8}
    & \textit{Front}
    & \textit{F.Left}
    & \textit{F.Right}
    & \textit{B.Left}
    & \textit{B.Right}
    & \textit{Back}
    & \textit{Avg.}
    \\
    \midrule
    Mono-Pre % glorious-grass-13154
    & 0.169
    & 0.203
    & 0.228
    & 0.235
    & 0.238
    & 0.206
    & 0.213 % .2131
    \\
    \midrule
    \textbf{\Acronym} % ANOVA
    & 0.161
    & \textbf{0.195}
    & \textbf{0.216}
    & \textbf{0.215}
    & \textbf{0.221}
    & 0.207
    & 0.202
    \\
    (stdev) % peachy-sun-13162, e=5
    & .001
    & .001
    & .001
    & .002
    & .001
    & .001
    & .020
    \\
    \midrule
    Mono* % peachy-sun-13162, e=5
    & 0.165
    & 0.196
    & 0.219
    & 0.216
    & 0.222
    & 0.209
    & 0.205
    \\
    (stdev) % peachy-sun-13162, e=5
    & .001
    & .000
    & .001
    & .002
    & .001
    & .002
    & .020
    \\
    % \midrule
    % FSM\textasteriskcentered % valiant-wind-13166, e=5
    % & 0.162
    % & 0.196
    % & 0.217
    % & 0.216
    % & 0.222
    % & 0.206
    % & 0.203
    % \\
    % (S.D.) % peachy-sun-13162, e=5
    % & .001
    % & .002
    % & .002
    % & .003
    % & .003
    % & .002
    % & .020
    % \\
    \midrule
    \midrule
    % Mono~\cite{packnet}
    % & -
    % & -
    % & -
    % & -
    % & -
    % & -
    % & -
    % \\
    FSM~\cite{fsm20222}
    & \textbf{0.130}
    & 0.201
    & 0.224
    & 0.229
    & 0.240
    & \textbf{0.186}
    & \textbf{0.201}
    \\
    \bottomrule
\end{tabular}
}
\caption{
\textbf{Scale-aware Depth estimation results} Mono-Pre is the backbone model (based on monodepth2~\cite{monodepth2} generated by the \emph{Scale-aware Pretraining}. \Acronym is Mono-Pre finetuned following the curriculum training procedure. Mono\textasteriskcentered\ is an ablation model of \Acronym; with predicted extrinsics removed. 
Note that FSM~\cite{fsm20222} uses ground truth extrinsics for training, while our model predicts.}
\label{tab:depth_ddad}
\vspace{-5mm}
\end{table}

==> tables/table_rot_averaging.tex <==
\captionsetup[table]{skip=6pt}

\begin{table}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{0.87}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|cccc}
\toprule
\textbf{Method} & 
Abs Rel$\downarrow$ &
Sq Rel$\downarrow$ &
RMSE$\downarrow$ &
$\delta_{1.25}$ $\uparrow$
\\
\toprule
FSM & 0.133 & 2.817 & \textbf{13.598} & 0.837\\
FSM + PCC (trans only) & 0.132 & 2.826 &  13.805 & 0.836\\
FSM + PCC (rot only) & 0.131 & 2.766 & 13.694 & 0.835 \\
\midrule
\textbf{FSM + PCC} & \textbf{0.130} & \textbf{2.752} & 13.866  & \textbf{0.838} \\
\bottomrule
\end{tabular}
}
\caption{
\textbf{Pose ablation (PCC)} described in Section 3.3. Our method with and without different components of the pose constraint, results on \textbf{F}.}
\label{table:pose-constraint}
\end{table}

==> tables/vs_colmap_extrinsics.tex <==
%Extrinsics Evaluation
\begin{table}%
% \vspace{-1mm}
\centering
\small
\renewcommand{\arraystretch}{1.00}
\setlength{\tabcolsep}{0.22em}
\subfloat[Translation error (Euclidean) \lbrack m\rbrack]{
\begin{tabular}{l|ccccc|c}
    \toprule
    \multirow{2}{*}{\textbf{Method}} &
    \multicolumn{6}{c}{$t\downarrow$} \\
    \cmidrule{2-7}
    & \textit{F.Left}
    & \textit{F.Right}
    & \textit{B.Left}
    & \textit{B.Right}
    & \textit{Back}
    & \textit{Avg.}
    \\
    \midrule
    COLMAP % (.105+.102+.104+.113+.066)/5
    & 0.105
    & 0.102
    & 0.104
    & 0.113
    & 0.066
    & 0.098
    \\
    \textbf{Self-FSM} % (0.050+0.051+0.074+0.062+0.071)/5
    & \textbf{0.050}
    & \textbf{0.051}
    & \textbf{0.074}
    & \textbf{0.062}
    & \textbf{0.071}
    & \textbf{0.062}
    \\
    \bottomrule
\end{tabular}
}
\\
\vspace{-2mm}
\subfloat[Translaiton error (Cosine similarity) \lbrack  \textdegree \rbrack]{
\begin{tabular}{l|ccccc|c}
    \toprule
    \multirow{2}{*}{\textbf{Method}} &
    \multicolumn{6}{c}{$t\downarrow$} \\
    \cmidrule{2-7}
    & \textit{F.Left}
    & \textit{F.Right}
    & \textit{B.Left}
    & \textit{B.Right}
    & \textit{Back}
    & \textit{Avg.}
    \\
    \midrule
    COLMAP
    & 32.44
    & 8.474
    & 4.828
    & 5.960
    & \textbf{2.367}
    & 10.81
    \\
    \textbf{Self-FSM}
    & \textbf{12.33}
    & \textbf{4.279}
    & \textbf{7.595}
    & \textbf{2.748}
    & 2.489
    & \textbf{5.888}
    \\
    \bottomrule
\end{tabular}
}
\\
\vspace{-2mm}
\subfloat[Rotation error (Geodesic) \lbrack  \textdegree \rbrack]{
\begin{tabular}{l|ccccc|c}
    \toprule
    \multirow{2}{*}{\textbf{Method}} &
    \multicolumn{6}{c}{$R\downarrow$} \\
    \cmidrule{2-7}    
    & \textit{F.Left}
    & \textit{F.Right}
    & \textit{B.Left}
    & \textit{B.Right}
    & \textit{Back}
    & \textit{Avg.}
    \\
    \midrule
    COLMAP % (0.010+0.016+.009+.027+.019)/5
    & 0.533
    & \textbf{0.208}
    & 0.485 
    & 1.029 
    & 0.445 
    & 0.540 
    \\
    \textbf{Self-FSM} % (0.024+.012+.016+.029+.012)/5 -> (degree)
    & \textbf{0.138}
    & 0.231
    & \textbf{0.152} 
    & \textbf{0.247}
    & \textbf{0.181}
    & \textbf{0.190}
    \\
    \bottomrule
\end{tabular}
}
% \vspace{-2mm}
\caption{\textbf{Extrinsics calibration performance on sequence 000052 of DDAD}. COLMAP output is scaled by the vehicle ego-motion.}
\label{tab:colmap1}
% \vspace{-3mm}
\end{table}

==> tables/vs_colmap_full_copy.tex <==
%Extrinsics Evaluation
%excel sheet: https://docs.google.com/spreadsheets/d/16hIHhuMsfnJ-7S6cIjnwnfgGvmDvQ-r4twX8_3xVb6A/edit#gid=739406365

% Under 1 meter
% - (Model I): fine-dawn-13464

% All
% - atomic-sunset-13465

\begin{table}%
\captionsetup[subfloat]{labelformat=empty} % Remove number from subfloat
% \vspace{-1mm}
\centering
\small
\renewcommand{\arraystretch}{1.00}
\setlength{\tabcolsep}{0.22em}
\subfloat{
\begin{tabular}{l|ccccc|c}
    \toprule
    \multirow{2}{*}{\textbf{Method}} &
    \multicolumn{6}{c}{$t$ \lbrack m\rbrack $\downarrow$} \\
    \cmidrule{2-7}
    & \textit{F.Left}
    & \textit{F.Right}
    & \textit{B.Left}
    & \textit{B.Right}
    & \textit{Back}
    & \textit{Avg.}
    \\
    \midrule
    COLMAP % (6.07+2.43+2.20+2.24+2.47)/5
    & 6.07 % 6.068
    & 2.43 % 2.434
    & 2.20 % 2.198
    & 2.24 % 2.240
    & 2.47 % 2.465
    & 3.08
    \\
    \textbf{Self-FSM}(\emph{I}) % (0.160+.240+.165+.268+.216)/5
    & 0.160
    & 0.240
    & 0.165
    & 0.268
    & 0.216
    & 0.210
    \\
    \bottomrule
\end{tabular}
}
\\
\subfloat[(a) Bundle adjustment (\emph{BA}) converged sequences (97/150)]{
\begin{tabular}{l|ccccc|c}
    \toprule
    \multirow{2}{*}{\textbf{Method}} &
    \multicolumn{6}{c}{$R$ \lbrack \textdegree \rbrack $\downarrow$} \\
    \cmidrule{2-7}    
    & \textit{F.Left}
    & \textit{F.Right}
    & \textit{B.Left}
    & \textit{B.Right}
    & \textit{Back}
    & \textit{Avg.}
    \\
    \midrule
    COLMAP % (2.01+1.61+1.73+1.75+1.12)/5
    & 2.01 % 2.011
    & 1.61 % 1.612
    & 1.73 % 1.727
    & 1.75 % 1.75
    & 1.12 % 1.196
    & 1.64
    \\
    \textbf{Self-FSM}(\emph{I}) % (1.60+1.96+1.05+2.57+1.48)/5
    & 1.60 % 1.603
    & 1.96 % 1.957
    & 1.05 % 1.047
    & 2.57 % 2.567
    & 1.48 % 1.475
    & 1.73
    \\
    \bottomrule
\end{tabular}
}
% \caption{November to April}
\\
\subfloat{
\begin{tabular}{l|ccccc|c}
    \toprule
    \multirow{2}{*}{\textbf{Method}} &
    \multicolumn{6}{c}{$t$ \lbrack m\rbrack $\downarrow$} \\
    \cmidrule{2-7}
    & \textit{F.Left}
    & \textit{F.Right}
    & \textit{B.Left}
    & \textit{B.Right}
    & \textit{Back}
    & \textit{Avg.}
    \\
    \midrule
    COLMAP % (.117+.282+.210+.308+.262)/5
    & 0.117
    & 0.282
    & 0.210
    & 0.308
    & 0.262
    & 0.236
    \\
    \textbf{Self-FSM}(\emph{I})% (0.150+0.225+0.158+0.260+0.206)/5
    & 0.150
    & 0.225
    & 0.158
    & 0.260
    & 0.206
    & 0.200
    \\
    \bottomrule
\end{tabular}
}
\\
\subfloat[(b) \emph{BA} converged and $t>1$ removed sequences (89/150))]{
\begin{tabular}{l|ccccc|c}
    \toprule
    \multirow{2}{*}{\textbf{Method}} &
    \multicolumn{6}{c}{$R$ \lbrack \textdegree \rbrack $\downarrow$} \\
    \cmidrule{2-7}    
    & \textit{F.Left}
    & \textit{F.Right}
    & \textit{B.Left}
    & \textit{B.Right}
    & \textit{Back}
    & \textit{Avg.}
    \\
    \midrule
    COLMAP% (1.25+0.873+1.02+0.937+0.434)/5
    & 1.25 % 1.251
    & 0.873 % 0.873
    & 1.02 % 1.016
    & 0.937 % 0.937
    & 0.434 % 0.434
    & 0.903
    \\
    \textbf{Self-FSM}(\emph{I}) % (1.67+1.95+1.07+2.57+1.44)/5
    & 1.67 % 1.672
    & 1.95 % 1.945
    & 1.07 % 1.071
    & 2.57 % 2.568
    & 1.44 % 1.441
    & 1.74 
    \\
    \bottomrule
\end{tabular}
}
% \vspace{-2mm}
\caption{\textbf{Extrinsic calibration performance on train split of DDAD}. COLMAP output is scaled by the vehicle odometry. Evaluation sequences are selected from the following conditions that (a) bundle adjustment (\emph{rig\_bundle\_adjuster}) process converged, (b) COLMAP "failing" scenario (the large translation error $t$ is larger than $1$[m]) are excluded. \emph{I} indicates the intrinsics learning model. 
}
\label{tab:full_colmap}
% \vspace{-3mm}
\end{table}
